Exact solutions for scalar field cosmology in f(R) gravity

We look for exact solutions in scalar field cosmology. To achieve this we use $f(R)$ modified gravity with a scalar field and do not specify the the form of the $f(R)$ function. In particular, we study Friedmann universe assuming that acceleration of the scalar curvature is negligible. We first present solutions for special cases and then the general solution. Using initial conditions which represent the universe at the present epoch, we evaluated the constants of integration. This allows for the comparison of the scale factor in the new solutions with that of the $\Lambda CDM$ solution, thereby affecting the age of the universe in $f(R)$ gravity.

==> figure0.tex <==
% GNUPLOT: LaTeX picture
\setlength{\unitlength}{0.240900pt}
\ifx\plotpoint\undefined\newsavebox{\plotpoint}\fi
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\begin{picture}(1500,900)(0,0)
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(755.0,131.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(755,90){\makebox(0,0){0}}
\put(755.0,839.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(983.0,131.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(983,90){\makebox(0,0){$t_*$}}
\put(983.0,839.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(71.0,131.0){\rule[-0.200pt]{0.400pt}{175.375pt}}
\put(71.0,131.0){\rule[-0.200pt]{329.551pt}{0.400pt}}
\put(1439.0,131.0){\rule[-0.200pt]{0.400pt}{175.375pt}}
\put(71.0,859.0){\rule[-0.200pt]{329.551pt}{0.400pt}}
\put(30,495){\makebox(0,0){$a_*$}}
\put(755,29){\makebox(0,0){t}}
\put(1279,819){\makebox(0,0)[r]{$a=a_*(|t-t_*|)^{1/2}$}}
\put(1299.0,819.0){\rule[-0.200pt]{24.090pt}{0.400pt}}
\put(71,859){\usebox{\plotpoint}}
\multiput(71.00,857.93)(1.214,-0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(71.00,858.17)(11.855,-6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(85.00,851.93)(1.489,-0.477){7}{\rule{1.220pt}{0.115pt}}
\multiput(85.00,852.17)(11.468,-5.000){2}{\rule{0.610pt}{0.400pt}}
\multiput(99.00,846.93)(1.123,-0.482){9}{\rule{0.967pt}{0.116pt}}
\multiput(99.00,847.17)(10.994,-6.000){2}{\rule{0.483pt}{0.400pt}}
\multiput(112.00,840.93)(1.489,-0.477){7}{\rule{1.220pt}{0.115pt}}
\multiput(112.00,841.17)(11.468,-5.000){2}{\rule{0.610pt}{0.400pt}}
\multiput(126.00,835.93)(1.214,-0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(126.00,836.17)(11.855,-6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(140.00,829.93)(1.214,-0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(140.00,830.17)(11.855,-6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(154.00,823.93)(1.214,-0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(154.00,824.17)(11.855,-6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(168.00,817.93)(1.214,-0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(168.00,818.17)(11.855,-6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(182.00,811.93)(1.378,-0.477){7}{\rule{1.140pt}{0.115pt}}
\multiput(182.00,812.17)(10.634,-5.000){2}{\rule{0.570pt}{0.400pt}}
\multiput(195.00,806.93)(1.214,-0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(195.00,807.17)(11.855,-6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(209.00,800.93)(1.214,-0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(209.00,801.17)(11.855,-6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(223.00,794.93)(1.214,-0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(223.00,795.17)(11.855,-6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(237.00,788.93)(1.026,-0.485){11}{\rule{0.900pt}{0.117pt}}
\multiput(237.00,789.17)(12.132,-7.000){2}{\rule{0.450pt}{0.400pt}}
\multiput(251.00,781.93)(1.123,-0.482){9}{\rule{0.967pt}{0.116pt}}
\multiput(251.00,782.17)(10.994,-6.000){2}{\rule{0.483pt}{0.400pt}}
\multiput(264.00,775.93)(1.214,-0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(264.00,776.17)(11.855,-6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(278.00,769.93)(1.214,-0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(278.00,770.17)(11.855,-6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(292.00,763.93)(1.026,-0.485){11}{\rule{0.900pt}{0.117pt}}
\multiput(292.00,764.17)(12.132,-7.000){2}{\rule{0.450pt}{0.400pt}}
\multiput(306.00,756.93)(1.214,-0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(306.00,757.17)(11.855,-6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(320.00,750.93)(1.026,-0.485){11}{\rule{0.900pt}{0.117pt}}
\multiput(320.00,751.17)(12.132,-7.000){2}{\rule{0.450pt}{0.400pt}}
\multiput(334.00,743.93)(1.123,-0.482){9}{\rule{0.967pt}{0.116pt}}
\multiput(334.00,744.17)(10.994,-6.000){2}{\rule{0.483pt}{0.400pt}}
\multiput(347.00,737.93)(1.026,-0.485){11}{\rule{0.900pt}{0.117pt}}
\multiput(347.00,738.17)(12.132,-7.000){2}{\rule{0.450pt}{0.400pt}}
\multiput(361.00,730.93)(1.026,-0.485){11}{\rule{0.900pt}{0.117pt}}
\multiput(361.00,731.17)(12.132,-7.000){2}{\rule{0.450pt}{0.400pt}}
\multiput(375.00,723.93)(1.214,-0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(375.00,724.17)(11.855,-6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(389.00,717.93)(1.026,-0.485){11}{\rule{0.900pt}{0.117pt}}
\multiput(389.00,718.17)(12.132,-7.000){2}{\rule{0.450pt}{0.400pt}}
\multiput(403.00,710.93)(0.950,-0.485){11}{\rule{0.843pt}{0.117pt}}
\multiput(403.00,711.17)(11.251,-7.000){2}{\rule{0.421pt}{0.400pt}}
\multiput(416.00,703.93)(1.026,-0.485){11}{\rule{0.900pt}{0.117pt}}
\multiput(416.00,704.17)(12.132,-7.000){2}{\rule{0.450pt}{0.400pt}}
\multiput(430.00,696.93)(1.026,-0.485){11}{\rule{0.900pt}{0.117pt}}
\multiput(430.00,697.17)(12.132,-7.000){2}{\rule{0.450pt}{0.400pt}}
\multiput(444.00,689.93)(0.890,-0.488){13}{\rule{0.800pt}{0.117pt}}
\multiput(444.00,690.17)(12.340,-8.000){2}{\rule{0.400pt}{0.400pt}}
\multiput(458.00,681.93)(1.026,-0.485){11}{\rule{0.900pt}{0.117pt}}
\multiput(458.00,682.17)(12.132,-7.000){2}{\rule{0.450pt}{0.400pt}}
\multiput(472.00,674.93)(1.026,-0.485){11}{\rule{0.900pt}{0.117pt}}
\multiput(472.00,675.17)(12.132,-7.000){2}{\rule{0.450pt}{0.400pt}}
\multiput(486.00,667.93)(0.824,-0.488){13}{\rule{0.750pt}{0.117pt}}
\multiput(486.00,668.17)(11.443,-8.000){2}{\rule{0.375pt}{0.400pt}}
\multiput(499.00,659.93)(1.026,-0.485){11}{\rule{0.900pt}{0.117pt}}
\multiput(499.00,660.17)(12.132,-7.000){2}{\rule{0.450pt}{0.400pt}}
\multiput(513.00,652.93)(0.890,-0.488){13}{\rule{0.800pt}{0.117pt}}
\multiput(513.00,653.17)(12.340,-8.000){2}{\rule{0.400pt}{0.400pt}}
\multiput(527.00,644.93)(0.890,-0.488){13}{\rule{0.800pt}{0.117pt}}
\multiput(527.00,645.17)(12.340,-8.000){2}{\rule{0.400pt}{0.400pt}}
\multiput(541.00,636.93)(0.890,-0.488){13}{\rule{0.800pt}{0.117pt}}
\multiput(541.00,637.17)(12.340,-8.000){2}{\rule{0.400pt}{0.400pt}}
\multiput(555.00,628.93)(0.824,-0.488){13}{\rule{0.750pt}{0.117pt}}
\multiput(555.00,629.17)(11.443,-8.000){2}{\rule{0.375pt}{0.400pt}}
\multiput(568.00,620.93)(0.890,-0.488){13}{\rule{0.800pt}{0.117pt}}
\multiput(568.00,621.17)(12.340,-8.000){2}{\rule{0.400pt}{0.400pt}}
\multiput(582.00,612.93)(0.786,-0.489){15}{\rule{0.722pt}{0.118pt}}
\multiput(582.00,613.17)(12.501,-9.000){2}{\rule{0.361pt}{0.400pt}}
\multiput(596.00,603.93)(0.890,-0.488){13}{\rule{0.800pt}{0.117pt}}
\multiput(596.00,604.17)(12.340,-8.000){2}{\rule{0.400pt}{0.400pt}}
\multiput(610.00,595.93)(0.786,-0.489){15}{\rule{0.722pt}{0.118pt}}
\multiput(610.00,596.17)(12.501,-9.000){2}{\rule{0.361pt}{0.400pt}}
\multiput(624.00,586.93)(0.786,-0.489){15}{\rule{0.722pt}{0.118pt}}
\multiput(624.00,587.17)(12.501,-9.000){2}{\rule{0.361pt}{0.400pt}}
\multiput(638.00,577.93)(0.728,-0.489){15}{\rule{0.678pt}{0.118pt}}
\multiput(638.00,578.17)(11.593,-9.000){2}{\rule{0.339pt}{0.400pt}}
\multiput(651.00,568.93)(0.786,-0.489){15}{\rule{0.722pt}{0.118pt}}
\multiput(651.00,569.17)(12.501,-9.000){2}{\rule{0.361pt}{0.400pt}}
\multiput(665.00,559.92)(0.704,-0.491){17}{\rule{0.660pt}{0.118pt}}
\multiput(665.00,560.17)(12.630,-10.000){2}{\rule{0.330pt}{0.400pt}}
\multiput(679.00,549.93)(0.786,-0.489){15}{\rule{0.722pt}{0.118pt}}
\multiput(679.00,550.17)(12.501,-9.000){2}{\rule{0.361pt}{0.400pt}}
\multiput(693.00,540.92)(0.704,-0.491){17}{\rule{0.660pt}{0.118pt}}
\multiput(693.00,541.17)(12.630,-10.000){2}{\rule{0.330pt}{0.400pt}}
\multiput(707.00,530.92)(0.652,-0.491){17}{\rule{0.620pt}{0.118pt}}
\multiput(707.00,531.17)(11.713,-10.000){2}{\rule{0.310pt}{0.400pt}}
\multiput(720.00,520.92)(0.637,-0.492){19}{\rule{0.609pt}{0.118pt}}
\multiput(720.00,521.17)(12.736,-11.000){2}{\rule{0.305pt}{0.400pt}}
\multiput(734.00,509.92)(0.637,-0.492){19}{\rule{0.609pt}{0.118pt}}
\multiput(734.00,510.17)(12.736,-11.000){2}{\rule{0.305pt}{0.400pt}}
\multiput(748.00,498.92)(0.637,-0.492){19}{\rule{0.609pt}{0.118pt}}
\multiput(748.00,499.17)(12.736,-11.000){2}{\rule{0.305pt}{0.400pt}}
\multiput(762.00,487.92)(0.637,-0.492){19}{\rule{0.609pt}{0.118pt}}
\multiput(762.00,488.17)(12.736,-11.000){2}{\rule{0.305pt}{0.400pt}}
\multiput(776.00,476.92)(0.582,-0.492){21}{\rule{0.567pt}{0.119pt}}
\multiput(776.00,477.17)(12.824,-12.000){2}{\rule{0.283pt}{0.400pt}}
\multiput(790.00,464.92)(0.539,-0.492){21}{\rule{0.533pt}{0.119pt}}
\multiput(790.00,465.17)(11.893,-12.000){2}{\rule{0.267pt}{0.400pt}}
\multiput(803.00,452.92)(0.536,-0.493){23}{\rule{0.531pt}{0.119pt}}
\multiput(803.00,453.17)(12.898,-13.000){2}{\rule{0.265pt}{0.400pt}}
\multiput(817.00,439.92)(0.536,-0.493){23}{\rule{0.531pt}{0.119pt}}
\multiput(817.00,440.17)(12.898,-13.000){2}{\rule{0.265pt}{0.400pt}}
\multiput(831.00,426.92)(0.497,-0.494){25}{\rule{0.500pt}{0.119pt}}
\multiput(831.00,427.17)(12.962,-14.000){2}{\rule{0.250pt}{0.400pt}}
\multiput(845.00,412.92)(0.497,-0.494){25}{\rule{0.500pt}{0.119pt}}
\multiput(845.00,413.17)(12.962,-14.000){2}{\rule{0.250pt}{0.400pt}}
\multiput(859.58,397.54)(0.493,-0.616){23}{\rule{0.119pt}{0.592pt}}
\multiput(858.17,398.77)(13.000,-14.771){2}{\rule{0.400pt}{0.296pt}}
\multiput(872.58,381.69)(0.494,-0.570){25}{\rule{0.119pt}{0.557pt}}
\multiput(871.17,382.84)(14.000,-14.844){2}{\rule{0.400pt}{0.279pt}}
\multiput(886.58,365.57)(0.494,-0.607){25}{\rule{0.119pt}{0.586pt}}
\multiput(885.17,366.78)(14.000,-15.784){2}{\rule{0.400pt}{0.293pt}}
\multiput(900.58,348.21)(0.494,-0.717){25}{\rule{0.119pt}{0.671pt}}
\multiput(899.17,349.61)(14.000,-18.606){2}{\rule{0.400pt}{0.336pt}}
\multiput(914.58,328.09)(0.494,-0.754){25}{\rule{0.119pt}{0.700pt}}
\multiput(913.17,329.55)(14.000,-19.547){2}{\rule{0.400pt}{0.350pt}}
\multiput(928.58,306.74)(0.494,-0.864){25}{\rule{0.119pt}{0.786pt}}
\multiput(927.17,308.37)(14.000,-22.369){2}{\rule{0.400pt}{0.393pt}}
\multiput(942.58,282.01)(0.493,-1.091){23}{\rule{0.119pt}{0.962pt}}
\multiput(941.17,284.00)(13.000,-26.004){2}{\rule{0.400pt}{0.481pt}}
\multiput(955.58,253.20)(0.494,-1.342){25}{\rule{0.119pt}{1.157pt}}
\multiput(954.17,255.60)(14.000,-34.598){2}{\rule{0.400pt}{0.579pt}}
\multiput(969.58,209.91)(0.494,-3.288){25}{\rule{0.119pt}{2.671pt}}
\multiput(968.17,215.46)(14.000,-84.455){2}{\rule{0.400pt}{1.336pt}}
\multiput(983.58,131.00)(0.494,3.288){25}{\rule{0.119pt}{2.671pt}}
\multiput(982.17,131.00)(14.000,84.455){2}{\rule{0.400pt}{1.336pt}}
\multiput(997.58,221.00)(0.494,1.342){25}{\rule{0.119pt}{1.157pt}}
\multiput(996.17,221.00)(14.000,34.598){2}{\rule{0.400pt}{0.579pt}}
\multiput(1011.58,258.00)(0.493,1.091){23}{\rule{0.119pt}{0.962pt}}
\multiput(1010.17,258.00)(13.000,26.004){2}{\rule{0.400pt}{0.481pt}}
\multiput(1024.58,286.00)(0.494,0.864){25}{\rule{0.119pt}{0.786pt}}
\multiput(1023.17,286.00)(14.000,22.369){2}{\rule{0.400pt}{0.393pt}}
\multiput(1038.58,310.00)(0.494,0.754){25}{\rule{0.119pt}{0.700pt}}
\multiput(1037.17,310.00)(14.000,19.547){2}{\rule{0.400pt}{0.350pt}}
\multiput(1052.58,331.00)(0.494,0.717){25}{\rule{0.119pt}{0.671pt}}
\multiput(1051.17,331.00)(14.000,18.606){2}{\rule{0.400pt}{0.336pt}}
\multiput(1066.58,351.00)(0.494,0.607){25}{\rule{0.119pt}{0.586pt}}
\multiput(1065.17,351.00)(14.000,15.784){2}{\rule{0.400pt}{0.293pt}}
\multiput(1080.58,368.00)(0.494,0.570){25}{\rule{0.119pt}{0.557pt}}
\multiput(1079.17,368.00)(14.000,14.844){2}{\rule{0.400pt}{0.279pt}}
\multiput(1094.58,384.00)(0.493,0.616){23}{\rule{0.119pt}{0.592pt}}
\multiput(1093.17,384.00)(13.000,14.771){2}{\rule{0.400pt}{0.296pt}}
\multiput(1107.00,400.58)(0.497,0.494){25}{\rule{0.500pt}{0.119pt}}
\multiput(1107.00,399.17)(12.962,14.000){2}{\rule{0.250pt}{0.400pt}}
\multiput(1121.00,414.58)(0.497,0.494){25}{\rule{0.500pt}{0.119pt}}
\multiput(1121.00,413.17)(12.962,14.000){2}{\rule{0.250pt}{0.400pt}}
\multiput(1135.00,428.58)(0.536,0.493){23}{\rule{0.531pt}{0.119pt}}
\multiput(1135.00,427.17)(12.898,13.000){2}{\rule{0.265pt}{0.400pt}}
\multiput(1149.00,441.58)(0.536,0.493){23}{\rule{0.531pt}{0.119pt}}
\multiput(1149.00,440.17)(12.898,13.000){2}{\rule{0.265pt}{0.400pt}}
\multiput(1163.00,454.58)(0.539,0.492){21}{\rule{0.533pt}{0.119pt}}
\multiput(1163.00,453.17)(11.893,12.000){2}{\rule{0.267pt}{0.400pt}}
\multiput(1176.00,466.58)(0.582,0.492){21}{\rule{0.567pt}{0.119pt}}
\multiput(1176.00,465.17)(12.824,12.000){2}{\rule{0.283pt}{0.400pt}}
\multiput(1190.00,478.58)(0.637,0.492){19}{\rule{0.609pt}{0.118pt}}
\multiput(1190.00,477.17)(12.736,11.000){2}{\rule{0.305pt}{0.400pt}}
\multiput(1204.00,489.58)(0.637,0.492){19}{\rule{0.609pt}{0.118pt}}
\multiput(1204.00,488.17)(12.736,11.000){2}{\rule{0.305pt}{0.400pt}}
\multiput(1218.00,500.58)(0.637,0.492){19}{\rule{0.609pt}{0.118pt}}
\multiput(1218.00,499.17)(12.736,11.000){2}{\rule{0.305pt}{0.400pt}}
\multiput(1232.00,511.58)(0.637,0.492){19}{\rule{0.609pt}{0.118pt}}
\multiput(1232.00,510.17)(12.736,11.000){2}{\rule{0.305pt}{0.400pt}}
\multiput(1246.00,522.58)(0.652,0.491){17}{\rule{0.620pt}{0.118pt}}
\multiput(1246.00,521.17)(11.713,10.000){2}{\rule{0.310pt}{0.400pt}}
\multiput(1259.00,532.58)(0.704,0.491){17}{\rule{0.660pt}{0.118pt}}
\multiput(1259.00,531.17)(12.630,10.000){2}{\rule{0.330pt}{0.400pt}}
\multiput(1273.00,542.59)(0.786,0.489){15}{\rule{0.722pt}{0.118pt}}
\multiput(1273.00,541.17)(12.501,9.000){2}{\rule{0.361pt}{0.400pt}}
\multiput(1287.00,551.58)(0.704,0.491){17}{\rule{0.660pt}{0.118pt}}
\multiput(1287.00,550.17)(12.630,10.000){2}{\rule{0.330pt}{0.400pt}}
\multiput(1301.00,561.59)(0.786,0.489){15}{\rule{0.722pt}{0.118pt}}
\multiput(1301.00,560.17)(12.501,9.000){2}{\rule{0.361pt}{0.400pt}}
\multiput(1315.00,570.59)(0.728,0.489){15}{\rule{0.678pt}{0.118pt}}
\multiput(1315.00,569.17)(11.593,9.000){2}{\rule{0.339pt}{0.400pt}}
\multiput(1328.00,579.59)(0.786,0.489){15}{\rule{0.722pt}{0.118pt}}
\multiput(1328.00,578.17)(12.501,9.000){2}{\rule{0.361pt}{0.400pt}}
\multiput(1342.00,588.59)(0.786,0.489){15}{\rule{0.722pt}{0.118pt}}
\multiput(1342.00,587.17)(12.501,9.000){2}{\rule{0.361pt}{0.400pt}}
\multiput(1356.00,597.59)(0.890,0.488){13}{\rule{0.800pt}{0.117pt}}
\multiput(1356.00,596.17)(12.340,8.000){2}{\rule{0.400pt}{0.400pt}}
\multiput(1370.00,605.59)(0.786,0.489){15}{\rule{0.722pt}{0.118pt}}
\multiput(1370.00,604.17)(12.501,9.000){2}{\rule{0.361pt}{0.400pt}}
\multiput(1384.00,614.59)(0.890,0.488){13}{\rule{0.800pt}{0.117pt}}
\multiput(1384.00,613.17)(12.340,8.000){2}{\rule{0.400pt}{0.400pt}}
\multiput(1398.00,622.59)(0.824,0.488){13}{\rule{0.750pt}{0.117pt}}
\multiput(1398.00,621.17)(11.443,8.000){2}{\rule{0.375pt}{0.400pt}}
\multiput(1411.00,630.59)(0.890,0.488){13}{\rule{0.800pt}{0.117pt}}
\multiput(1411.00,629.17)(12.340,8.000){2}{\rule{0.400pt}{0.400pt}}
\multiput(1425.00,638.59)(0.890,0.488){13}{\rule{0.800pt}{0.117pt}}
\multiput(1425.00,637.17)(12.340,8.000){2}{\rule{0.400pt}{0.400pt}}
\put(71.0,131.0){\rule[-0.200pt]{0.400pt}{175.375pt}}
\put(71.0,131.0){\rule[-0.200pt]{329.551pt}{0.400pt}}
\put(1439.0,131.0){\rule[-0.200pt]{0.400pt}{175.375pt}}
\put(71.0,859.0){\rule[-0.200pt]{329.551pt}{0.400pt}}
\end{picture}


==> figure2_0.tex <==
% GNUPLOT: LaTeX picture
\setlength{\unitlength}{0.240900pt}
\ifx\plotpoint\undefined\newsavebox{\plotpoint}\fi
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\begin{picture}(1500,900)(0,0)
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(755.0,131.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(755,90){\makebox(0,0){0}}
\put(755.0,839.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1211.0,131.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(1211,90){\makebox(0,0){$t_*$}}
\put(1211.0,839.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(71.0,131.0){\rule[-0.200pt]{0.400pt}{175.375pt}}
\put(71.0,131.0){\rule[-0.200pt]{329.551pt}{0.400pt}}
\put(1439.0,131.0){\rule[-0.200pt]{0.400pt}{175.375pt}}
\put(71.0,859.0){\rule[-0.200pt]{329.551pt}{0.400pt}}
\put(30,495){\makebox(0,0){$a_*$}}
\put(755,29){\makebox(0,0){t}}
\put(1279,819){\makebox(0,0)[r]{$a=a_*(|\cos(\sqrt{2}\mu (t_*-t))|)^{1/2}$}}
\put(1299.0,819.0){\rule[-0.200pt]{24.090pt}{0.400pt}}
\put(71,131){\usebox{\plotpoint}}
\multiput(71.58,131.00)(0.494,7.144){25}{\rule{0.119pt}{5.671pt}}
\multiput(70.17,131.00)(14.000,183.229){2}{\rule{0.400pt}{2.836pt}}
\multiput(85.58,326.00)(0.494,2.921){25}{\rule{0.119pt}{2.386pt}}
\multiput(84.17,326.00)(14.000,75.048){2}{\rule{0.400pt}{1.193pt}}
\multiput(99.58,406.00)(0.493,2.400){23}{\rule{0.119pt}{1.977pt}}
\multiput(98.17,406.00)(13.000,56.897){2}{\rule{0.400pt}{0.988pt}}
\multiput(112.58,467.00)(0.494,1.819){25}{\rule{0.119pt}{1.529pt}}
\multiput(111.17,467.00)(14.000,46.827){2}{\rule{0.400pt}{0.764pt}}
\multiput(126.58,517.00)(0.494,1.562){25}{\rule{0.119pt}{1.329pt}}
\multiput(125.17,517.00)(14.000,40.242){2}{\rule{0.400pt}{0.664pt}}
\multiput(140.58,560.00)(0.494,1.305){25}{\rule{0.119pt}{1.129pt}}
\multiput(139.17,560.00)(14.000,33.658){2}{\rule{0.400pt}{0.564pt}}
\multiput(154.58,596.00)(0.494,1.195){25}{\rule{0.119pt}{1.043pt}}
\multiput(153.17,596.00)(14.000,30.835){2}{\rule{0.400pt}{0.521pt}}
\multiput(168.58,629.00)(0.494,1.011){25}{\rule{0.119pt}{0.900pt}}
\multiput(167.17,629.00)(14.000,26.132){2}{\rule{0.400pt}{0.450pt}}
\multiput(182.58,657.00)(0.493,0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(181.17,657.00)(13.000,22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(195.58,681.00)(0.494,0.754){25}{\rule{0.119pt}{0.700pt}}
\multiput(194.17,681.00)(14.000,19.547){2}{\rule{0.400pt}{0.350pt}}
\multiput(209.58,702.00)(0.494,0.644){25}{\rule{0.119pt}{0.614pt}}
\multiput(208.17,702.00)(14.000,16.725){2}{\rule{0.400pt}{0.307pt}}
\multiput(223.58,720.00)(0.494,0.534){25}{\rule{0.119pt}{0.529pt}}
\multiput(222.17,720.00)(14.000,13.903){2}{\rule{0.400pt}{0.264pt}}
\multiput(237.00,735.58)(0.637,0.492){19}{\rule{0.609pt}{0.118pt}}
\multiput(237.00,734.17)(12.736,11.000){2}{\rule{0.305pt}{0.400pt}}
\multiput(251.00,746.59)(0.728,0.489){15}{\rule{0.678pt}{0.118pt}}
\multiput(251.00,745.17)(11.593,9.000){2}{\rule{0.339pt}{0.400pt}}
\multiput(264.00,755.59)(1.214,0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(264.00,754.17)(11.855,6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(278.00,761.61)(2.918,0.447){3}{\rule{1.967pt}{0.108pt}}
\multiput(278.00,760.17)(9.918,3.000){2}{\rule{0.983pt}{0.400pt}}
\multiput(306.00,762.95)(2.918,-0.447){3}{\rule{1.967pt}{0.108pt}}
\multiput(306.00,763.17)(9.918,-3.000){2}{\rule{0.983pt}{0.400pt}}
\multiput(320.00,759.93)(1.214,-0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(320.00,760.17)(11.855,-6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(334.00,753.93)(0.728,-0.489){15}{\rule{0.678pt}{0.118pt}}
\multiput(334.00,754.17)(11.593,-9.000){2}{\rule{0.339pt}{0.400pt}}
\multiput(347.00,744.92)(0.637,-0.492){19}{\rule{0.609pt}{0.118pt}}
\multiput(347.00,745.17)(12.736,-11.000){2}{\rule{0.305pt}{0.400pt}}
\multiput(361.58,732.81)(0.494,-0.534){25}{\rule{0.119pt}{0.529pt}}
\multiput(360.17,733.90)(14.000,-13.903){2}{\rule{0.400pt}{0.264pt}}
\multiput(375.58,717.45)(0.494,-0.644){25}{\rule{0.119pt}{0.614pt}}
\multiput(374.17,718.73)(14.000,-16.725){2}{\rule{0.400pt}{0.307pt}}
\multiput(389.58,699.09)(0.494,-0.754){25}{\rule{0.119pt}{0.700pt}}
\multiput(388.17,700.55)(14.000,-19.547){2}{\rule{0.400pt}{0.350pt}}
\multiput(403.58,677.52)(0.493,-0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(402.17,679.26)(13.000,-22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(416.58,653.26)(0.494,-1.011){25}{\rule{0.119pt}{0.900pt}}
\multiput(415.17,655.13)(14.000,-26.132){2}{\rule{0.400pt}{0.450pt}}
\multiput(430.58,624.67)(0.494,-1.195){25}{\rule{0.119pt}{1.043pt}}
\multiput(429.17,626.84)(14.000,-30.835){2}{\rule{0.400pt}{0.521pt}}
\multiput(444.58,591.32)(0.494,-1.305){25}{\rule{0.119pt}{1.129pt}}
\multiput(443.17,593.66)(14.000,-33.658){2}{\rule{0.400pt}{0.564pt}}
\multiput(458.58,554.48)(0.494,-1.562){25}{\rule{0.119pt}{1.329pt}}
\multiput(457.17,557.24)(14.000,-40.242){2}{\rule{0.400pt}{0.664pt}}
\multiput(472.58,510.65)(0.494,-1.819){25}{\rule{0.119pt}{1.529pt}}
\multiput(471.17,513.83)(14.000,-46.827){2}{\rule{0.400pt}{0.764pt}}
\multiput(486.58,458.79)(0.493,-2.400){23}{\rule{0.119pt}{1.977pt}}
\multiput(485.17,462.90)(13.000,-56.897){2}{\rule{0.400pt}{0.988pt}}
\multiput(499.58,396.10)(0.494,-2.921){25}{\rule{0.119pt}{2.386pt}}
\multiput(498.17,401.05)(14.000,-75.048){2}{\rule{0.400pt}{1.193pt}}
\multiput(513.58,302.46)(0.494,-7.144){25}{\rule{0.119pt}{5.671pt}}
\multiput(512.17,314.23)(14.000,-183.229){2}{\rule{0.400pt}{2.836pt}}
\multiput(527.58,131.00)(0.494,7.144){25}{\rule{0.119pt}{5.671pt}}
\multiput(526.17,131.00)(14.000,183.229){2}{\rule{0.400pt}{2.836pt}}
\multiput(541.58,326.00)(0.494,2.921){25}{\rule{0.119pt}{2.386pt}}
\multiput(540.17,326.00)(14.000,75.048){2}{\rule{0.400pt}{1.193pt}}
\multiput(555.58,406.00)(0.493,2.400){23}{\rule{0.119pt}{1.977pt}}
\multiput(554.17,406.00)(13.000,56.897){2}{\rule{0.400pt}{0.988pt}}
\multiput(568.58,467.00)(0.494,1.819){25}{\rule{0.119pt}{1.529pt}}
\multiput(567.17,467.00)(14.000,46.827){2}{\rule{0.400pt}{0.764pt}}
\multiput(582.58,517.00)(0.494,1.562){25}{\rule{0.119pt}{1.329pt}}
\multiput(581.17,517.00)(14.000,40.242){2}{\rule{0.400pt}{0.664pt}}
\multiput(596.58,560.00)(0.494,1.305){25}{\rule{0.119pt}{1.129pt}}
\multiput(595.17,560.00)(14.000,33.658){2}{\rule{0.400pt}{0.564pt}}
\multiput(610.58,596.00)(0.494,1.195){25}{\rule{0.119pt}{1.043pt}}
\multiput(609.17,596.00)(14.000,30.835){2}{\rule{0.400pt}{0.521pt}}
\multiput(624.58,629.00)(0.494,1.011){25}{\rule{0.119pt}{0.900pt}}
\multiput(623.17,629.00)(14.000,26.132){2}{\rule{0.400pt}{0.450pt}}
\multiput(638.58,657.00)(0.493,0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(637.17,657.00)(13.000,22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(651.58,681.00)(0.494,0.754){25}{\rule{0.119pt}{0.700pt}}
\multiput(650.17,681.00)(14.000,19.547){2}{\rule{0.400pt}{0.350pt}}
\multiput(665.58,702.00)(0.494,0.644){25}{\rule{0.119pt}{0.614pt}}
\multiput(664.17,702.00)(14.000,16.725){2}{\rule{0.400pt}{0.307pt}}
\multiput(679.58,720.00)(0.494,0.534){25}{\rule{0.119pt}{0.529pt}}
\multiput(678.17,720.00)(14.000,13.903){2}{\rule{0.400pt}{0.264pt}}
\multiput(693.00,735.58)(0.637,0.492){19}{\rule{0.609pt}{0.118pt}}
\multiput(693.00,734.17)(12.736,11.000){2}{\rule{0.305pt}{0.400pt}}
\multiput(707.00,746.59)(0.728,0.489){15}{\rule{0.678pt}{0.118pt}}
\multiput(707.00,745.17)(11.593,9.000){2}{\rule{0.339pt}{0.400pt}}
\multiput(720.00,755.59)(1.214,0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(720.00,754.17)(11.855,6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(734.00,761.61)(2.918,0.447){3}{\rule{1.967pt}{0.108pt}}
\multiput(734.00,760.17)(9.918,3.000){2}{\rule{0.983pt}{0.400pt}}
\put(292.0,764.0){\rule[-0.200pt]{3.373pt}{0.400pt}}
\multiput(762.00,762.95)(2.918,-0.447){3}{\rule{1.967pt}{0.108pt}}
\multiput(762.00,763.17)(9.918,-3.000){2}{\rule{0.983pt}{0.400pt}}
\multiput(776.00,759.93)(1.214,-0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(776.00,760.17)(11.855,-6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(790.00,753.93)(0.728,-0.489){15}{\rule{0.678pt}{0.118pt}}
\multiput(790.00,754.17)(11.593,-9.000){2}{\rule{0.339pt}{0.400pt}}
\multiput(803.00,744.92)(0.637,-0.492){19}{\rule{0.609pt}{0.118pt}}
\multiput(803.00,745.17)(12.736,-11.000){2}{\rule{0.305pt}{0.400pt}}
\multiput(817.58,732.81)(0.494,-0.534){25}{\rule{0.119pt}{0.529pt}}
\multiput(816.17,733.90)(14.000,-13.903){2}{\rule{0.400pt}{0.264pt}}
\multiput(831.58,717.45)(0.494,-0.644){25}{\rule{0.119pt}{0.614pt}}
\multiput(830.17,718.73)(14.000,-16.725){2}{\rule{0.400pt}{0.307pt}}
\multiput(845.58,699.09)(0.494,-0.754){25}{\rule{0.119pt}{0.700pt}}
\multiput(844.17,700.55)(14.000,-19.547){2}{\rule{0.400pt}{0.350pt}}
\multiput(859.58,677.52)(0.493,-0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(858.17,679.26)(13.000,-22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(872.58,653.26)(0.494,-1.011){25}{\rule{0.119pt}{0.900pt}}
\multiput(871.17,655.13)(14.000,-26.132){2}{\rule{0.400pt}{0.450pt}}
\multiput(886.58,624.67)(0.494,-1.195){25}{\rule{0.119pt}{1.043pt}}
\multiput(885.17,626.84)(14.000,-30.835){2}{\rule{0.400pt}{0.521pt}}
\multiput(900.58,591.32)(0.494,-1.305){25}{\rule{0.119pt}{1.129pt}}
\multiput(899.17,593.66)(14.000,-33.658){2}{\rule{0.400pt}{0.564pt}}
\multiput(914.58,554.48)(0.494,-1.562){25}{\rule{0.119pt}{1.329pt}}
\multiput(913.17,557.24)(14.000,-40.242){2}{\rule{0.400pt}{0.664pt}}
\multiput(928.58,510.65)(0.494,-1.819){25}{\rule{0.119pt}{1.529pt}}
\multiput(927.17,513.83)(14.000,-46.827){2}{\rule{0.400pt}{0.764pt}}
\multiput(942.58,458.79)(0.493,-2.400){23}{\rule{0.119pt}{1.977pt}}
\multiput(941.17,462.90)(13.000,-56.897){2}{\rule{0.400pt}{0.988pt}}
\multiput(955.58,396.10)(0.494,-2.921){25}{\rule{0.119pt}{2.386pt}}
\multiput(954.17,401.05)(14.000,-75.048){2}{\rule{0.400pt}{1.193pt}}
\multiput(969.58,302.46)(0.494,-7.144){25}{\rule{0.119pt}{5.671pt}}
\multiput(968.17,314.23)(14.000,-183.229){2}{\rule{0.400pt}{2.836pt}}
\multiput(983.58,131.00)(0.494,7.144){25}{\rule{0.119pt}{5.671pt}}
\multiput(982.17,131.00)(14.000,183.229){2}{\rule{0.400pt}{2.836pt}}
\multiput(997.58,326.00)(0.494,2.921){25}{\rule{0.119pt}{2.386pt}}
\multiput(996.17,326.00)(14.000,75.048){2}{\rule{0.400pt}{1.193pt}}
\multiput(1011.58,406.00)(0.493,2.400){23}{\rule{0.119pt}{1.977pt}}
\multiput(1010.17,406.00)(13.000,56.897){2}{\rule{0.400pt}{0.988pt}}
\multiput(1024.58,467.00)(0.494,1.819){25}{\rule{0.119pt}{1.529pt}}
\multiput(1023.17,467.00)(14.000,46.827){2}{\rule{0.400pt}{0.764pt}}
\multiput(1038.58,517.00)(0.494,1.562){25}{\rule{0.119pt}{1.329pt}}
\multiput(1037.17,517.00)(14.000,40.242){2}{\rule{0.400pt}{0.664pt}}
\multiput(1052.58,560.00)(0.494,1.305){25}{\rule{0.119pt}{1.129pt}}
\multiput(1051.17,560.00)(14.000,33.658){2}{\rule{0.400pt}{0.564pt}}
\multiput(1066.58,596.00)(0.494,1.195){25}{\rule{0.119pt}{1.043pt}}
\multiput(1065.17,596.00)(14.000,30.835){2}{\rule{0.400pt}{0.521pt}}
\multiput(1080.58,629.00)(0.494,1.011){25}{\rule{0.119pt}{0.900pt}}
\multiput(1079.17,629.00)(14.000,26.132){2}{\rule{0.400pt}{0.450pt}}
\multiput(1094.58,657.00)(0.493,0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(1093.17,657.00)(13.000,22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(1107.58,681.00)(0.494,0.754){25}{\rule{0.119pt}{0.700pt}}
\multiput(1106.17,681.00)(14.000,19.547){2}{\rule{0.400pt}{0.350pt}}
\multiput(1121.58,702.00)(0.494,0.644){25}{\rule{0.119pt}{0.614pt}}
\multiput(1120.17,702.00)(14.000,16.725){2}{\rule{0.400pt}{0.307pt}}
\multiput(1135.58,720.00)(0.494,0.534){25}{\rule{0.119pt}{0.529pt}}
\multiput(1134.17,720.00)(14.000,13.903){2}{\rule{0.400pt}{0.264pt}}
\multiput(1149.00,735.58)(0.637,0.492){19}{\rule{0.609pt}{0.118pt}}
\multiput(1149.00,734.17)(12.736,11.000){2}{\rule{0.305pt}{0.400pt}}
\multiput(1163.00,746.59)(0.728,0.489){15}{\rule{0.678pt}{0.118pt}}
\multiput(1163.00,745.17)(11.593,9.000){2}{\rule{0.339pt}{0.400pt}}
\multiput(1176.00,755.59)(1.214,0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(1176.00,754.17)(11.855,6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(1190.00,761.61)(2.918,0.447){3}{\rule{1.967pt}{0.108pt}}
\multiput(1190.00,760.17)(9.918,3.000){2}{\rule{0.983pt}{0.400pt}}
\put(748.0,764.0){\rule[-0.200pt]{3.373pt}{0.400pt}}
\multiput(1218.00,762.95)(2.918,-0.447){3}{\rule{1.967pt}{0.108pt}}
\multiput(1218.00,763.17)(9.918,-3.000){2}{\rule{0.983pt}{0.400pt}}
\multiput(1232.00,759.93)(1.214,-0.482){9}{\rule{1.033pt}{0.116pt}}
\multiput(1232.00,760.17)(11.855,-6.000){2}{\rule{0.517pt}{0.400pt}}
\multiput(1246.00,753.93)(0.728,-0.489){15}{\rule{0.678pt}{0.118pt}}
\multiput(1246.00,754.17)(11.593,-9.000){2}{\rule{0.339pt}{0.400pt}}
\multiput(1259.00,744.92)(0.637,-0.492){19}{\rule{0.609pt}{0.118pt}}
\multiput(1259.00,745.17)(12.736,-11.000){2}{\rule{0.305pt}{0.400pt}}
\multiput(1273.58,732.81)(0.494,-0.534){25}{\rule{0.119pt}{0.529pt}}
\multiput(1272.17,733.90)(14.000,-13.903){2}{\rule{0.400pt}{0.264pt}}
\multiput(1287.58,717.45)(0.494,-0.644){25}{\rule{0.119pt}{0.614pt}}
\multiput(1286.17,718.73)(14.000,-16.725){2}{\rule{0.400pt}{0.307pt}}
\multiput(1301.58,699.09)(0.494,-0.754){25}{\rule{0.119pt}{0.700pt}}
\multiput(1300.17,700.55)(14.000,-19.547){2}{\rule{0.400pt}{0.350pt}}
\multiput(1315.58,677.52)(0.493,-0.933){23}{\rule{0.119pt}{0.838pt}}
\multiput(1314.17,679.26)(13.000,-22.260){2}{\rule{0.400pt}{0.419pt}}
\multiput(1328.58,653.26)(0.494,-1.011){25}{\rule{0.119pt}{0.900pt}}
\multiput(1327.17,655.13)(14.000,-26.132){2}{\rule{0.400pt}{0.450pt}}
\multiput(1342.58,624.67)(0.494,-1.195){25}{\rule{0.119pt}{1.043pt}}
\multiput(1341.17,626.84)(14.000,-30.835){2}{\rule{0.400pt}{0.521pt}}
\multiput(1356.58,591.32)(0.494,-1.305){25}{\rule{0.119pt}{1.129pt}}
\multiput(1355.17,593.66)(14.000,-33.658){2}{\rule{0.400pt}{0.564pt}}
\multiput(1370.58,554.48)(0.494,-1.562){25}{\rule{0.119pt}{1.329pt}}
\multiput(1369.17,557.24)(14.000,-40.242){2}{\rule{0.400pt}{0.664pt}}
\multiput(1384.58,510.65)(0.494,-1.819){25}{\rule{0.119pt}{1.529pt}}
\multiput(1383.17,513.83)(14.000,-46.827){2}{\rule{0.400pt}{0.764pt}}
\multiput(1398.58,458.79)(0.493,-2.400){23}{\rule{0.119pt}{1.977pt}}
\multiput(1397.17,462.90)(13.000,-56.897){2}{\rule{0.400pt}{0.988pt}}
\multiput(1411.58,396.10)(0.494,-2.921){25}{\rule{0.119pt}{2.386pt}}
\multiput(1410.17,401.05)(14.000,-75.048){2}{\rule{0.400pt}{1.193pt}}
\multiput(1425.58,302.46)(0.494,-7.144){25}{\rule{0.119pt}{5.671pt}}
\multiput(1424.17,314.23)(14.000,-183.229){2}{\rule{0.400pt}{2.836pt}}
\put(1204.0,764.0){\rule[-0.200pt]{3.373pt}{0.400pt}}
\put(71.0,131.0){\rule[-0.200pt]{0.400pt}{175.375pt}}
\put(71.0,131.0){\rule[-0.200pt]{329.551pt}{0.400pt}}
\put(1439.0,131.0){\rule[-0.200pt]{0.400pt}{175.375pt}}
\put(71.0,859.0){\rule[-0.200pt]{329.551pt}{0.400pt}}
\end{picture}

